SciFive: a text-to-text transformer model for biomedical literature

In this report, we introduce SciFive, a domain-specific T5 model that has been pre-trained on large biomedical corpora. Our model outperforms the current SOTA methods (i.e. BERT, BioBERT, Base T5) on tasks in named entity relation, relation extraction, natural language inference, and question-answering. We show that text-generation methods have significant potential in a broad array of biomedical NLP tasks, particularly those requiring longer, more complex outputs. Our results support the exploration of more difficult text generation tasks and the development of new methods in this area

==> section/scifive.tex <==
SciFive follows the sequence-to-sequence encoder-decoder architecture proposed by \cite{DBLP:journals/corr/VaswaniSPUJGKP17} and the T5 framework released by \cite{DBLP:journals/corr/abs-1910-10683}. The original T5 work implemented five different model size - Small, Base, Large, 3B, and 11B. For the purpose of this study and computation limitation, we will use the base and large model in this research, with 220 million parameters and 770 million parameters respectively.

==> section/supervised.tex <==
\subsection{Supervised Tasks and Datasets}
In this work, we trained 14 supervised tasks in the biomedical text domain describe below:
\subsubsection{Named-Entity Regconition (NER)}
\textbf{NCBI disease corpus} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{BC5CDR} (Disease and Chemical annotations):

\textbf{BC4CHEMD} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{BC2GM} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{JNLPBA} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{Species-800} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{Chem Rot} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{DDI} \citep{doan2014disease}: a corpus with 792 texts originating from the DrugBank database. It also consists of 233 Medline abstracts. 

DDI extraction 2013 corpus is a collection of 792 texts selected from the DrugBank database and other 233 Medline abstracts (Herrero-Zazo et al., 2013).5 The drug-drug interactions, includ- ing both pharmacokinetic and pharmacodynamic interactions, were annotated by two expert phar- macists with a substantial background in pharma- covigilance. In our benchmark, we use 624 train files and 191 test files to evaluate the performance and report the micro-average F1-score of the four DDI types.

\textbf{HoC} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{MedNLI} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{bioasq4b} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{bioasq5b} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

\textbf{bioasq6b} \citep{doan2014disease}: a resource for disease name recognition with disease annotators from 793 PubMed abstracts and 6,892 disease mentions for the biomedical natural language processing community. The dataset is available with train, valid, and test set.

==> table/ner_result.tex <==
\begin{table*}[]
\begin{tabular}{@{}clllccc@{}}
\toprule
Task                                     & Dataset         & Entity type          & Number of entities   & Task Type                             & Input Length         & Target Length        \\ \midrule
\multirow{3}{*}{Self-Supervise Learning} & PubMed          & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{\multirow{3}{*}{}} & 1024                 & 1024                 \\
                                         & PMC             & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{}                  & 1024                 & 1024                 \\
                                         & PubMed+PMC      & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{}                  & 1024                 & 1024                 \\ \midrule
\multirow{7}{*}{Name-entity Recognition} & NCBI Disease    & Disease              & 6881                 & \multirow{7}{*}{Multi-Task}           & \multirow{7}{*}{512} & \multirow{7}{*}{512} \\
                                         & BC5CDR Disease  & Disease              & 19,665               &                                       &                      &                      \\
                                         & BC5CDR Chem     & Disease              & 12,694               &                                       &                      &                      \\
                                         & BC4CHEMD        & Chemical                 & 15,411               &                                       &                      &                      \\
                                         & BC2HM           & Chemical                 & 79,842               &                                       &                      &                      \\
                                         & JNLPBA          & Gene                 & 20,703               &                                       &                      &                      \\
                                         & Species-800     & Species              & 3708                 &                                       &                      &                      \\ \midrule
Relational Extraction                    & Chemprot        & Protein-chemical     & 10,031               & Single-Task                           & 256                  & 16                   \\
                                         & DDI             & Biomedical relation  & 4,920                & Single-Task                           & 256                  & 16                   \\ \midrule
Document classification                  & HoC             & Biomedical Documents & 1,580                & Single-Task                           & 256                  & 64                   \\ \midrule
Inference                                & MedNLI          & Clinical pairs       & 14,049               & Single-Task                           & 256                  & 12                   \\ \midrule
\multirow{3}{*}{Question Answering}      & BioASQ4-factoid & Biomedical QA        & 488                  & Single-Task                           & 512                  & 128                  \\
                                         & BioASQ5-factoid & Biomedical QA        & 636                  & Single-Task                           & 512                  & 128                  \\
                                         & BioASQ6-factoid & Biomedical QA        & 779                  & Single-Task                           & 512                  & 128                  \\ \bottomrule
\end{tabular}
\label{ner_result}
\end{table*}
